Atiyah-Floer Conjecture: a Formulation, a Strategy to Prove and Generalizations

Around 1988, Floer introduced two important theories: instanton Floer homology as invariants of 3-manifolds and Lagrangian Floer homology as invariants of pairs of Lagrangians in symplectic manifolds. Soon after that, Atiyah conjectured that the two theories should be related to each other and Lagrangian Floer homology of certain Lagrangians in the moduli space of flat connections on Riemann surfaces should recover instanton Floer homology. However, the space of flat connections on a Riemann surface is singular and the first step to address this conjecture is to make sense of Lagrangian Floer homology on this space. In this note, we formulate a possible approach to resolve this issue. A strategy to construct the desired isomorphism in the Atiyah-Floer conjecture is also sketched. We also use the language of A infty-categories to state generalizations of the Atiyah-Floer conjecture.

==> divisor-comp.tex <==
%!TEX root = proceeding.tex

\section{Lagrangian Floer Theory in a Smooth Divisor Complement}\label{sec:divisor complement}

%{\color{red} Introductory Paragraph}
%In order to use the cut down extended moduli space in the definition of symplectic instanton Floer homology, we need to clarify how we treat the non-compactness of the extended moduli space. If we compactify the extended moduli space naively, then the symplectic form degenerates at infinity. In \cite{MW}, symplectic cuts of the extended moduli space is employed to obtain compact symplectic manifolds. See Sections \ref{sec:extendedmoduli} and \ref{sec:generalgroup}. In the case $G=SU(2)$, we can proceed as follows. \marginpar{\color{red}The introduction paragraph needs to be modified to motivate Lagrangian Floer homology in the divisor complements}

Let $(X,\omega)$ be a compact 
symplctic manifold and $D$ be a codimension $2$ submanimfold. We assume that $(X,D)$ is a K\"ahler manifold in a neighborhood of $D$, and $D$ is a smooth divisor in this neighborhood. 
\begin{definition}
	Let $L_1$ and $L_2$ be compact subsets of $X\setminus D$.
	We say $L_1$ is {\it Hamiltonian isotopic} to $L_2$ relative to $D$ 
	if there exists a compactly supported time dependent Hamiltonian 
	$H : (X\backslash D) \times [0,1] \to \R$ so that the Hamiltonian diffeomorphism $\varphi : X \setminus D \to X \setminus D$
	generated by $H$ sends $L_1$ to $L_2$, that is, $\varphi(L_1) = L_2$.
\end{definition}
\begin{definition}
	We say $L \subset X \setminus D$ is {\it monotone} if 
	\eqref{ineq32} holds for $\beta \in H_2(X\setminus D,L)$.
	The minimal Maslov number of $L$ relative to $D$ is defined as:
	\[
	  \inf \{\mu_L(\beta) \mid \beta \in \pi_2(X\setminus D,L),\,\omega(\beta) >0 \}.
	\]	
\end{definition}

\begin{theorem}\label{mainthm}
{\rm (\cite{DF})}
	Let $L_0,L_1$ be compact, monotone and spin Lagrangian submanifolds of $X\setminus D$.	
	We assume that {\rm (m.a)} or {\rm (m.b)} holds for these Lagrangains.
	Then there is a vector space $HF(L_0,L_1;X\setminus D)$ over $\Q$ which is called 
	the Lagrangian Floer homology of $L_0$ and $L_1$ relative to $D$, and satisfies the following properties:
	\vspace{-5pt}
	\begin{enumerate}
	\item[(i)]
		If $L_0$ is transversal to $L_1$ then we have
		$$
		{\rm rank}_{\Q} HF(L_0,L_1;X\setminus D) \le \# (L_0 \cap L_1).
		$$
	\item[(ii)]
		If $L_i'$ is Hamiltonian isotopic to $L_i$ in $X \setminus D$ 
		for $i=0,1$ then
		$$
		HF(L_0,L_1;X\setminus D) \cong HF(L'_0,L'_1;X\setminus D)
		$$
	\item[(iii)]
		If $L_0 = L_1 =L$ and {\rm (m.a)} holds, then there exists a 
		spectral sequence whose $E^2$ page is  $H(L;\Q)$
		and which converges to $HF(L,L;X\setminus D)$. \marginpar{\color{red} Should we state this part about clean intersections?}
	\end{enumerate}
\end{theorem}
\begin{remark}
	The main point in Theorem \ref{mainthm} is that 
	we do {\it not} assume $L_i$ is a monotone Lagrangian submanifold 
	in $X$, for $i=1,2$. The general theory of \cite{fooobook,fooobook2}
	says that there is an obstruction to define Floer homology $HF(L_0,L_1)$.
	The Floer homology $HF(L_0,L_1;X\setminus D)$ uses only holomorphic disks 
	which `do not intersect' $D$. Therefore, the situation is similar to
	monotone Lagrangian Floer homology due to Oh \cite{Oh}.
	If $X\setminus D$ is convex at infinity, then \cite{fooobook,fooobook2} imply 
	that we can define Floer homology $HF(L_0,L_1;X\setminus D)$ satisfying the properties mentioned in Theorem \ref{mainthm}.
	Note that in Theorem \ref{mainthm}, we do not impose any kind of convexity assumption for $X \setminus D$.
	The specialization of the construction of Theorem \ref{mainthm} to the case that $L_i$ 
	is exact and the homology class of each component of $D$ is proportional to the Poincar\'e dual 
	of $[\omega]$ is given in \cite{sh}.
	
%\begin{enumerate}
%\item
%We can continue and construct $A_{\infty}$ category whose object is a monotone 
%Lagrangian submanifold $L$ in $X\setminus D$.
%\item
%Actually we can define Floer homology over $\Z$ coefficient, 
%using monotonicity and \cite{fooooverZ}.
%See Remark \ref{remrem6767}.
%\item
%We use $\R$ coefficient since we use de Rham theory to work out the 
%transversality issue during the proof following 
%\cite{fooo:tech2-1,fooo:tech2-2}, 
%in Sections \ref{boundaryope} and ???.
%\end{enumerate}
\end{remark}

\begin{proof}[Sketch of the proof]
	We assume that $L_0$ is transversal to $L_1$. Let $p,q \in L_0 \cap L_1$. We consider the moduli space
	$\overset{\circ}{\mathcal M}(p,q;\beta;L_0,L_1)$ of pseudo-holomorphic maps to $X\backslash D$
	which satisfy \eqref{CR} and \eqref{form38} for $G=\{1\}$. Following Floer \cite{Fl:LHF} and Oh \cite{Oh} 
	(see also \cite[Chapter2]{fooobook}), we can define $HF(L_0,L_1;X\setminus D)$ 
	if we obtain a compactification ${\mathcal M}^{\rm RGW}(p,q;\beta;L_0,L_1)$ of our moduli space 
	$\overset{\circ}{\mathcal M}(p,q;\beta;L_0,L_1)$ with the following properties:
\begin{enumerate}
	\item[(I)] The compactification ${\mathcal M}^{\rm RGW}(p,q;\beta;L_0,L_1)$ 
	 carries a Kuranishi structure with boundary and corner.
	\item[(II)] The codimension one boundary of this moduli space is identified with the union of 
		\begin{equation}\label{splitend} 
		{\mathcal M}^{\rm RGW}(p,r;\beta_1;L_0,L_1) \times 
		{\mathcal M}^{\rm RGW}(r,q;\beta_2;L_0,L_1)
	\end{equation}
	for various $r \in L_1 \cap L_2$ and $\beta_1,\beta_2$
	with $\beta_1 + \beta_2 = \beta$. The (virtual) dimension $d(\beta)$ of ${\mathcal M}^{\rm RGW}(p,q;\beta;L_0,L_1)$
	is determined by the homology class $\beta$ and satisfies $d(\beta) = d(\beta_1) + d(\beta_2) + 1$ 
	for the boundary component in \eqref{splitend}.
\end{enumerate}
	We fix a {\it multisection}\footnote{See \cite[Definition A1.21]{fooobook2})} (or equivalently a multivalued perturbation) 
	which is transversal to $0$ and which is compatible with the description of the boundary as in \eqref{splitend}.
	Note that transversality implies that its zero set is the empty set when the virtual dimension is negative.
	Therefore, the zero set is a finite set in the case that the virtual dimension is $0$.
	Assuming $d(\beta) = 0$, let $\# {\mathcal M}^{\rm RGW}(p,q;\beta;L_0,L_1)$ 
	be the number (counted with sign and multiplicity) of the
	points in the zero set of the perturbed moduli space. Then we define:
	\[
	  \partial [p] = \sum_{q,\beta} \# {\mathcal M}^{\rm RGW}(p,q;\beta;L_0,L_1)[q].
	\]
	Here the sum is taken over all $q \in L_0 \cap L_1$ and the homology classes $\beta$ such that $d(\beta) = 0$. 
	The properties of  compactification imply that the right hand side is actually a finite sum.
	As it is customary with other Floer theories, we can show $\partial\circ \partial = 0$ using the moduli spaces associated to the homology classes $\beta$
	 with $d(\beta) =1$. (See, for example, \cite{Fl:LHF,Oh}.) The proofs of parts $(ii)$ and $(iii)$) are also similar to the 
	 proof of the corresponding statements in the case of usual monotone Lagrangian Floer homology.
	
 
	The stable map compactification in \cite[Subsection 7.1.4]{fooobook2} does {\it not} give a compactification 
	${\mathcal M}^{\rm RGW}(p,q;\beta;L_0,L_1)$ with the required properties.
	The issue is that in the stable map compactification a stable map with a sphere bubble which 
	is contained completely in the divisor $D$ is included.
	 {\color{red} At the point of such stable maps, 
	 the limit of the following two kinds of sequence of stable maps mixed up.
	\begin{enumerate}
	\item[(a)] 
		A limit of a sequence of pseudo-holomorphic disks $u_i : (D^2,\partial D^2) \to (X,L)$
		such that $u_i(D^2) \cap D = \emptyset$.
	\item[(b)]
		A limit of a sequence of stable maps $u_i : (\Sigma_i,\partial \Sigma_i) \to (X,L)$,
		where $\Sigma_i$ is a disk plus sphere bubbles, 
		and such that $u_i(\Sigma_i) \cap D \ne \emptyset$.
	\end{enumerate}
	We need to include (a) in our moduli space but (b) is not supposed to be 
	an element of the moduli space.

	If $X\setminus D$ is convex the above phenomenon cannot occur. 
	We can avoid this trouble by dimension counting if, for any 
	nontr	ivial holomorphic map $v : S^2 \to D$, the inequality
	$v_*([S^2]) \cap D > 0$ holds. In general it is hard to avoid it using the stable 
	map compactification.

	The idea to resolve this issue is to use a compactification 
	which is different from the stable map compactification (in $X$).
	We use the compactification used in relative 
	Gromov-Witten theory, where the 
	limits of type (a) and type (b) are clearly separated. (See \cite{IP,LR,pa,TZ}.)
	We can then show the above properties (I)(II).}
\end{proof}
	

%\section{Langrangian Floer Theory in a Smooth Divisor Complement}\label{sec:divisor complement}
%
%In order to use the extended moduli space in the definition of symplectic instanton Floer homology, we need to clarify how we treat the non-compactness of the extended moduli space. If we compactify the extended moduli space naively, then the symplectic form degenerates at infinity. The idea (which was already mentioned by \cite{MW}) is to use symplectic cut to obtain a compact  symplectic manifold. See Sections \ref{sec:extendedmoduli} and \ref{sec:generalgroup}. In the case $G=SU(2)$, we can work proceed as follows. 
%
%Let $(X,\omega)$ be a compact 
%symplctic manifold and $D$ is a codimension $2$ submanimfold. We assume that $(X,D)$ is a K\"ahler manifold in a neighborhood of $D$ and $D$ is a smooth divisor in this neighborhood. For a Lagrangian submanifold $L$ of $X$ we denote the Maslov index by ${\rm ms} : H_2(X,L;\Z) \to \Z$.\footnote{See \cite[Definition 2.1.15]{fooobook}.}
%\begin{definition}
%	A Lagrangian submanifold $L$ is {\it monotone in $X\setminus D$}, if there exists $c>0$ such that the following identity holds for 
%	all $\beta \in {\rm Im}(\pi_2(X\setminus D,L) \to \pi_2(X,L))$:
%        \begin{equation}
%        		c\cdot {\rm ms}(\beta) = \omega(\beta).
%        \end{equation}
%\end{definition}
%\begin{definition}
%	The {\it minimal Maslov number of $L \subset X \setminus D$} is defined to be:
%	\begin{equation}
%		\inf \{{\rm ms}(\beta) \mid \beta \in {\rm Im}(\pi_2(X\setminus D,L) \to \pi_2(X,L)),\,\omega(\beta) >0 \}.
%	\end{equation}
%\end{definition}
%\begin{definition}
%	Let $L_1$ and $L_2$ be be compact subsets of $X\setminus D$.
%	We say $L_1$ is {\it Hamiltonian isotopic} to $L_2$ if there exists a compactly supported time dependent Hamiltonian 
%	$H : (X\backslash D) \times [0,1] \to \R$ so that the Hamiltonian diffeomorphism $\varphi : X \setminus D \to X \setminus D$
%	generated by $H$ sends $L_1$ to $L_2$, that is, $\varphi(L_1) = L_2$.
%\end{definition}
%%Here $\varphi$ is defined from $H$ as follows.
%%We put $H_t(x) = H(x,t)$. Let $X_{H_t}$ be the Hamiltonian 
%%vector field associated to $H_t$. We define $\varphi^t$ by 
%%$$
%%\varphi^0(x) = x, 
%%\qquad
%%\frac{d}{dt}\varphi^t = X_{H_t} \circ \varphi^t.
%%$$
%%We put $\varphi = \varphi^1$.
%%\par
%%We say that $\varphi$ is a {\it Hamiltonian diffeomorphism 
%%associated to the (non-autonomous) Hamiltonian $H$}.
%%\par
%%The main result of this paper is the following.
%
%\begin{theorem}\label{mainthm}
%{\rm (\cite{DF})}
%	Let $L_0,L_1$ be compact, monotone and spin Lagrangian submanifolds of $X\setminus D$ with minimal Maslov numbers
%	We assume that one of the following conditions holds:
%	\begin{enumerate}
%	\item[(a)]
%		The minimal Maslov numbers of $L_0$ and of $L_1$ are both strictly greater than 2.
%	\item[(b)]
%		The Lagrangian submanifold $L_1$  is Hamiltonian isotopic to $L_0$. 
%	\end{enumerate}
%	Then we can define Lagrangian Floer homology group $HF(L_0,L_1;X\setminus D)$,
%	that is a $\Q$ vector space,
%	and satisfies the following properties.
%	\begin{enumerate}
%	\item
%		If $L_0$ is transversal to $L_1$ then we have
%		$$
%		{\rm rank}_{\Q} HF(L_0,L_1;X\setminus D) \le \# (L_0 \cap L_1).
%		$$
%	\item
%		If $L_i'$ is Hamiltonian isotopic to $L_i$ in $X \setminus D$ 
%		for $i=0,1$ then
%		$$
%		HF(L_0,L_1;X\setminus D) \cong HF(L'_0,L'_1;X\setminus D)
%		$$
%	\item
%		If $L_0 = L_1 =L$ and Case (a) holds, then we have:
%		$$
%		HF(L,L;X\setminus D) \cong H(L;\Q)
%		$$
%		where the right hand side is the singular homology group of $L$.
%		(In Case (b), there exists a spectral sequence similar to \cite{Oh2,fooobook,Bi}.)
%	\end{enumerate}
%\end{theorem}
%\begin{remark}
%	We remark that in Theorem \ref{mainthm}
%	we do {\it not} assume that $L_i$ is a monotone Lagrangian submanifold 
%	in $X$, for $i=1,2$. The general theory of \cite{fooobook,fooobook2}
%	says that there is an obstruction to define Floer homology $HF(L_0,L_1)$.
%	The Floer homology $HF(L_0,L_1;X\setminus D)$ uses only holomorphic disks 
%	which `do not intersect' $D$. Therefore the situation is similar to the 
%	monotone Floer homology due to Oh \cite{Oh}.
%	
%	In the case $X\setminus D$ is convex at infinity, \cite{fooobook,fooobook2} implies 
%	that we can define Floer homology $HF(L_0,L_1;X\setminus D)$ satisfying the properties mentioned in Theorem \ref{mainthm}.
%	Note that in Theorem \ref{mainthm}, we do not impose any kind of convexity assumption for $X \setminus D$.
%	In the case $L_i$ is exact and the homology class of each component of $D$ is proportional to the Poincar\'e dual 
%	to the cohomology class of  the symplectic form $[\omega]$, Theorem \ref{mainthm} is also a part of Sheridan's construction \cite{sh}.
%	
%\begin{enumerate}
%\item
%We can continue and construct $A_{\infty}$ category whose object is a monotone 
%Lagrangian submanifold $L$ in $X\setminus D$.
%\item
%Actually we can define Floer homology over $\Z$ coefficient, 
%using monotonicity and \cite{fooooverZ}.
%See Remark \ref{remrem6767}.
%%\item
%%We use $\R$ coefficient since we use de Rham theory to work out the 
%%transversality issue during the proof following 
%%\cite{fooo:tech2-1,fooo:tech2-2}, 
%%in Sections \ref{boundaryope} and ???.
%\end{enumerate}
%\end{remark}
%\begin{remark}
%	In Theorem \ref{mainthm} we assumed $L_i$ is spin, for $i=1,2$.
%We can relax this condition to the condition that 
%$(L_0,L_1)$ is a relatively spin pair in $X\setminus D$.
%(See \cite[Definition 3.1.1]{fooobook} for the definition of relatively spin pair.)
%\end{remark}
%\begin{proof}[Sketch of the proof]
%We assume that $L_0$ is transversal to $L_1$. 
%Let $p,q \in L_0 \cap L_1$. 
%We consider a homology class $\beta$ of maps
%$u : \R \times [0,1] \to X$ such that
%\begin{enumerate}
%\item
%$u(\R \times \{0\}) \subset L_0$,
%$u(\R \times \{1\}) \subset L_1$.
%\item
%$\lim_{\tau\to+\infty} u(\tau,t) = q$.
%$\lim_{\tau\to-\infty} u(\tau,t) = p$.
%\end{enumerate}
%We consider the moduli space 
%$\overset{\circ}{\mathcal M}(p,q;\beta;L_0,L_1)$
%of pseudo-holomorphic maps
%$u : \R \times [0,1] \to X \setminus D$
%with the above boundary conditions.
%(We moreover identify two maps $u$ and $u'$ if 
%$u'(\tau,t) = u(\tau+\tau_0,t)$ for some 
%$\tau_0 \in \R$.)
%Following the proof of Floer \cite{Flo88IV} and Oh \cite{Oh} 
%(See also \cite[Chapter2]{fooobook}.)
%we can define $HF(L_0,L_1;X\setminus D)$ 
%if we prove the following.
%\begin{enumerate}
%\item[(I)]
%There exists a compactification 
%${\mathcal M}^{\rm RGW}(p,q;\beta;L_0,L_1)$
%of our moduli space 
%$\overset{\circ}{\mathcal M}(p,q;\beta;L_0,L_1)$, 
%which carries a Kuranishi structure with boundary and corner.
%\item[(II)]
%The boundary of this moduli space is identified with the union of 
%\begin{equation}\label{splitend}
%{\mathcal M}^{\rm RGW}(p,r;\beta_1;L_0,L_1)
%\times 
%{\mathcal M}^{\rm RGW}(r,q;\beta_2;L_0,L_1)
%\end{equation}
%for various $r \in L_1 \cap L_2$ and $\beta_1,\beta_2$
%with $\beta_1 + \beta_2 = \beta$.
%\end{enumerate}
%The (virtual) dimension $d(\beta)$ of ${\mathcal M}^{\rm RGW}(p,q;\beta;L_0,L_1)$
%is determined by the homology class $\beta$ and satisfies
%$d(\beta) = d(\beta_1) + d(\beta_2) + 1$ in the situation of 
%(\ref{splitend}).
%\par
%We take a multisection 
%(multivalued perturbation. See \cite[Definition A1.21]{fooobook2}) 
%which is transversal to $0$ and which is compatible 
%with the description of the boundary as in (\ref{splitend}).
%Note transversality implies that its zero set is the empty set 
%in case when the virtual dimension is negative.
%Therefore (\ref{splitend}) implies that 
%the zero set is a finite set in case when the virtual dimension is $0$.
%We define
%$
%\# {\mathcal M}(p,q;\beta;L_0,L_1)
%$
%as the number (counted with sign and multiplicity) of the zero set of 
%the perturbed moduli space ${\mathcal M}(p,q;\beta;L_0,L_1)$,
%in case $d(\beta) = 0$.
%We then put
%$$
%\partial [p] = \sum_{q,\beta} \# {\mathcal M}(p,q;\beta;L_0,L_1)[q].
%$$
%Note the sum is taken over all $q \in L_0 \cap L_1$ and the homology class $\beta$ such that 
%$d(\beta) = 0$. We remark by monotonicity and Gromov compactness
%the right hand side is actually a finite sum.
%\par
%Then using the case $d(\beta) =1$ and (\ref{splitend})
%we can prove $\partial\circ \partial = 0$ in the same way as 
%\cite{Flo88IV,Oh}.
%\par
%The proof of Statements (2)(3) is also similar to the 
%proof of corresponding statements in the case of usual 
%monotone Lagrangian Floer homology.
%\par
%We remark however that the stable map compactification 
%in \cite[Subsection 7.1.4]{fooobook2} 
%does {\it not} give a compactification ${\mathcal M}^{\rm RGW}(p,q;\beta;L_0,L_1)$
%with required properties.
%The issue is that in the stable map compactification 
%a stable map with a sphere bubble which 
%is contained completely in the divisor $D$ is included.
%At the point of such stable maps, 
%the limit of the following two kinds of sequence 
%of stable maps mixed up.
%\begin{enumerate}
%\item[(a)] 
%A limit of a sequence of pseudo-holomorphic disks $u_i : (D^2,\partial D^2) \to (X,L)$
%such that $u_i(D^2) \cap D = \emptyset$.
%\item[(b)]
%A limit of a sequence of stable maps $u_i : (\Sigma_i,\partial \Sigma_i) \to (X,L)$,
%where $\Sigma_i$ is a disk plus sphere bubbles, 
%and such that $u_i(\Sigma_i) \cap D \ne \emptyset$.
%\end{enumerate}
%We need to include (a) in our moduli space but (b) is not supposed to be 
%an element of the moduli space.
%\par
%If $X\setminus D$ is convex the above phenomenon cannot occur. 
%We can avoid this trouble by dimension counting if, for any 
%nontrivial holomorphic map $v : S^2 \to D$, the inequality
%$v_*([S^2]) \cap D > 0$ holds. In general it is hard to avoid it using the stable 
%map compactification.
%\par
%The idea to resolve this issue is to use a compactification 
%which is different from the stable map compactification (in $X$).
%We use the compactification used in relative 
%Gromov-Witten theory, where the 
%limits of type (a) and type (b) are clearly separated. (See \cite{IP,LR,pa,TZ}.)
%We can then show the above properties (I)(II).
%\end{proof}
%We can combine Theorem \ref{mainthm} with the story of Section \ref{sec:equivariant}.
%We consider the next situation (which is one we use in the 
%next section.)
%
%\begin{shitu}\label{shitu66}
%Let $(X,\omega)$ be a symplectic manifold with $G$ action.
%Let $\frak L$ be a clean collection on $G$ invariant 
%and spin 
%immersed Lagrangian 
%submanifolds. We assume:
%\begin{enumerate}
%\item
%The $G$ action on $(X,\omega)$
%has a moment map
%$$
%\mu : X \to \frak g^*.
%$$
%\item
%If $L \in \frak L$ then $L \subset \mu^{-1}(0)$.
%\item
%The subspace $D$ is a codimension $2$ submanimfold of $X$.
%We assume that $(X,\omega,J)$ is a K\"ahler manifold in 
%a neighborhood of $D$ and 
%$D$ is its smooth divisor.
%\item
%The divisor $D$ is $G$ invariant.
%\item
%We require $D \cap \mu^{-1}(0) = \emptyset$.
%\end{enumerate}
%\end{shitu}
%\begin{theorem}\label{thm6767}
%In Situation \ref{shitu66} the following holds.
%\begin{enumerate}
%\item
%For an element $L$ of $\frak L$ we can define a 
%structure $\{\frak m_k^G\}$ of (curved) 
%filtered $A_{\infty}$ algebra on 
%$H_G(L;\Lambda_0)$. 
%\item
%In case $G=\{1\}$ and $L$ is monotone in $X \setminus D$ we have 
%$\frak m^G_0 = 0$
%and the $\frak m^G_1$ homology coincides with $HF(L,L; X\setminus D)$
%in Theorem \ref{mainthm}.
%\item
%We can define a filtered $A_{\infty}$ category
%$\frak{Fuk}(\frak L,X\setminus D,G)$,
%whose object is a pair $(L,b)$ of 
%an element $L$ of $\frak L$ and the bounding cochain 
%$b$ of the filtered $A_{\infty}$ algebra in Item (1).
%\item
%Suppose the action of $G$ is free on $\mu^{-1}(0)$ and we put $Y = 
%\mu^{-1}(0)/G$. We define $\overline{\frak L}$ as in (\ref{Lbar}).
%Moreover we assume (\ref{quotcorr}) is spin.
%\par
%Then there exists $\frak b \in H^{\rm even}(Y;\Lambda_+)$
%such that $\frak{Fuk}(\frak L,X\setminus D,G)$ is 
%homotopy equivalent to $\frak{Fuk}(\overline{\frak L},Y,\frak b)$.
%\par
%If (\ref{quotcorr}) is monotone with minimal Maslov number $>2$ in 
%addition then $\frak b = 0$.
%\end{enumerate}
%\end{theorem}
%Note the filtered $A_{\infty}$ structure in Item (1) is different 
%from those we obtain in Theorem \ref{thm54}.
%In Theorem \ref{thm6767} we use a compactification of 
%the moduli space of pseudo-holomorphic disks in $X \setminus D$
%which bounds $L$.
%On the other hand, in Theorem \ref{thm54} we use 
%all the holomorphic disks in $X$ which bounds $L$ 
%to define our operators.
%\begin{remark}
%We also remark that the Lagrangian submanifold appearing in 
%Theorem \ref{thm6767} is in general obstructed. Namely 
%$\frak m_0^G \ne 0$. In particular Floer homology 
%among them may not be defined. 
%The obstruction theory in \cite{fooobook} applies 
%and Floer homology is defined among the pairs $(L,b)$ of 
%Lagrangian submanifold $L$ and its  
%bounding cochain $b$.
%\end{remark}
%\begin{conjecture}\label{cong59}
%Theorems \ref{mainthm}, \ref{thm6767} still hold in case 
%$D$ is not necessary smooth but is normal crossing.
%\end{conjecture}
%\begin{remark}
%	It is plausible that the compactification appearing in relative Gromov-Witten theory for the complements of normal crossing divisors
%	can be employed to prove Conjecture \ref{cong59}. The analysis of Gromov-Witten theory for the complement of normal crossing
%	divisors is much harder than the case of complements of smooth divisors, and we would expect that a similar phenomena happen 
%	for Lagrangian Floer homology.
%\end{remark}
%	
